ASID: Active Exploration for System Identification in Robotic Manipulation

Model-free control strategies such as reinforcement learning have shown the ability to learn control strategies without requiring an accurate model or simulator of the world. While this is appealing due to the lack of modeling requirements, such methods can be sample inefficient, making them impractical in many real-world domains. On the other hand, model-based control techniques leveraging accurate simulators can circumvent these challenges and use a large amount of cheap simulation data to learn controllers that can effectively transfer to the real world. The challenge with such model-based techniques is the requirement for an extremely accurate simulation, requiring both the specification of appropriate simulation assets and physical parameters. This requires considerable human effort to design for every environment being considered. In this work, we propose a learning system that can leverage a small amount of real-world data to autonomously refine a simulation model and then plan an accurate control strategy that can be deployed in the real world. Our approach critically relies on utilizing an initial (possibly inaccurate) simulator to design effective exploration policies that, when deployed in the real world, collect high-quality data. We demonstrate the efficacy of this paradigm in identifying articulation, mass, and other physical parameters in several challenging robotic manipulation tasks, and illustrate that only a small amount of real-world data can allow for effective sim-to-real transfer. Project website at https://weirdlabuw.github.io/asid

==> apdx/reconstruction.tex <==
\subsubsection{Scene Reconstruction}
\awcomment{we said in one of our rebuttals that ``we will move the paragraph on the reconstruction pipeline (Section 4.2.2) to the experimental evaluation (Section 5.)''. I'm inclined to say we still move to the appendix as we discussed, but wanted to mention this}

Besides its physical parameters, a scene's geometry and kinematic tree are essential for many downstream applications that go beyond isolated object manipulation. However, these properties cannot be inferred by classical state-based system identification techniques. To include them in our simulator reconstruction, we turn to recent developments in vision-based scene reconstruction.
%To nonetheless include them in our simulator reconstruction and show the generality of \asid, we turn to recent developments in vision-based scene reconstruction.

%We record RGB and depth observation for the rollouts trajectory $\trajreal$ and leverage recent developments in scene reconstruction techniques.

% To stress generality, we consider environments that don't simply identify physical parameters like mass or friction but also the structure of the kinematic tree such as articulation and joint positioning. 
%  shit on SfA, ditto in the house, etc.

%\awcomment{it might be helpful to add some more rationale as to why we are doing the scene reconstruction as it's not mentioned before this point. In particular, with how we've presented the method up to this point, we're suggesting that we just need to learn $\btheta$, but this suggests that we actually need to learn other stuff too. If this is an important part, it might be worth mentioning earlier}

In particular, we collect RGB and depth in our rollout trajectory $\trajreal$ and compute pointclouds using the intrinsic and extrinsic parameters of two calibrated cameras.
By subtracting the first and last observation of each trajectory, we can separate moving and static parts of the scene, assuming the object of interest was moved during exploration. Inspired by \cite{byravan2022nerf2real}, we decompose the static parts of the scene into convex hulls---we use CoACD~\citep{wei2022approximate} for the decomposition---allowing for collision detection in simulation. The moving parts can then act as initialization for downstream tracking pipelines.
While several off-the-shelf components for articulated joint and part inference exist, they require before- and after-snapshots of the object. To get these, most works turn to movement primitives~\citep{nie2022structure,ma2023sim2real2} or manually moving the articulated object~\citep{Hsu2023DittoITH}. The proposed exploration, maximizing the Fisher information, can act as a learned replacement for such hand-designed techniques.

\awcomment{R2 had the following comment I was not sure how to address (also relevant when RANSAC is mentioned in experiments):

``This is maybe just me being pedantic, but frame/point cloud detection is not tracking. Tracking requires some sequential estimation. Note that this is not a critique on the section: continuous detection might be enough for the experiments. However, as before with the model-based RL it is a suggestion on proper naming conventions to clarify the text.''
}

==> tabs/sim_laptop_articulation.tex <==
\begin{table}[t]
\centering
\caption{Generated by Spread-LaTeX}\label{tab: }
\scriptsize
    \begin{tabular}{lc}\toprule
    Method & Success/Trials \\
    \midrule
    Random exploration & $1/5$ \\
    \cite{kumar2019estimating} & $0/5$ \\
    \glsentryshort{asid} (ours) & $4/5$  \\
    \bottomrule
\end{tabular}
\end{table}
